Verification of a real-time ensemble-based method for updating earth model based on GAN

The complexity of geomodelling workflows is a limiting factor for quantifying and updating uncertainty in real-time during drilling. We propose Generative Adversarial Networks (GANs) for parametrization and generation of geomodels, combined with Ensemble Randomized Maximum Likelihood (EnRML) for rapid updating of subsurface uncertainty. This real-time ensemble method combined with a highly non-linear model arising from neural-network modeling sequences might produce inaccurate and/or biased posterior solutions. This paper illustrates the predictive ability of EnRML on several examples where we assimilate local extra-deep electromagnetic logs. Statistical verification with MCMC confirms that the proposed workflow can produce reliable results required for geosteering wells.

==> highlights.tex <==
\section*{Highlights}
\todo{Create 3-5 highlights}
\begin{itemize}
    \item We demonstrated a real-time data assimilation for geosteering based on neural networks
    \item Generative-adversarial-network geomodel helps handle complex geology
    \item The small Gaussian GAN pasteurization is easier to update with ensemble method
    \item The neural networks help offload the computational burdon from real-time operation to training
    \item Real-time EnRML approximates the reference MCMC posterior during geosteering
\end{itemize}

==> plan.tex <==

\section{Plan}
\begin{itemize}
    \item Training (good input images, should we add faults)
    \item Set up things in python code (to work with anything EM)
\end{itemize}

\subsection{Plan June 3}

\begin{itemize}
    \item[Sergey] Check variance for different logs from the training
    \item[Kristian] Reduce variance in prior / synthetic truth to 1e-2
    \item[Sergey] Set up best GAN based on Jan's input
    \subitem Check the ranges of ML inputs. Make them in the range of ML.
    \subitem Put a reasonable Archie's Law. 
    \item[Kristian] Visualization again 
    \subitem heat map of variance / std of resistivity in each pixel
    \item[Sergey] fix get resistivity default to get resistivity
\end{itemize}

\subsection{Plan May 25}

{\bf Goal: The ideal scenario if we can detect structure ahead-of-bit}
     

\begin{itemize}
    \item [Kristian] Assimilate step-wise going column by column
    \item [Kristian] Set up a meaningful synthetic truth and upload it to REPO, fix a seed
    \item [Kristian] Do some visualization / validation? 
    \subitem Reduction in STD in image space behind the bit
    \subitem Almost the same STD in image space ahead
    \subitem Plot STD image == show variation in each pixel (do channel by channel)?
    \item [Sergey] Train and set-up the right GAN (the best we have)
    \item [Sergey] Make a converter from 6-channel pixel to resistivity
\end{itemize}


\subsection{Training}
    Generate something that can support a straight channel.
    
    Should we filter the GAN output?
    
    Linear point-wise update. Facies-type id tool
    
    Gamma log? 
    
    EM log?
    
    Let's make a model that we can pick up.
    
    Extra GAN to color with resistivity?
    
    Stochastic realization of resestivities from facies one per facies type.
    
\section{What to do}
    Jan checks resistivites in the images of fluvial.
    For final output (64x64 image needs to be meaningfull
    640 meters in length
    32 meters meters)
    
    The cell size (10m x 0.5m)
    
    Training image (4km x 1000m x 200m) 400x1x400
    4 facies for now
    
    Jan needs to writes about how the sedimentary system for training is created
    
    Jan can check the EM properties of facies
    
    We need a function to populate the model with properties
    
\section{Start with EnKF}
    Forward simulator in python
    
    Lets drill like that
    \begin{verbatim}
    xoxoxooxoxoxxoox
    xxoxooxoxoxxxoox
    ---->xoxoxoxoxox
    oxoxoxoxooxoxxoo
    oxoxoxoxooxoxxoo
    \end{verbatim}


